Intelligent Router for LLM Workloads: Improving Performance Through Workload-Aware Load Balancing

Large Language Model (LLM) workloads have distinct prefill and decode phases with different compute and memory requirements which should ideally be accounted for when scheduling input queries across different LLM instances in a cluster. However existing scheduling algorithms treat LLM workloads as monolithic jobs without considering the distinct characteristics of the two phases in each workload. This leads to sub-optimal scheduling and increased response latency. In this work, we start by characterizing factors affecting the response latency during LLM inference serving. We establish that better load balancing of inference requests across the available LLM instances can improve the end-to-end latency to a larger extent than merely focusing on optimizing the instance-level scheduler. Motivated by our findings, we propose a heuristic-guided reinforcement learning-based intelligent router for data-driven and workload-aware scheduling. Our router schedules queries across LLM instances by leveraging a trainable response-length predictor, and a novel formulation for estimating the impact of mixing different workloads and achieves over 11% lower end-to-end latency than existing approaches on a mix of public datasets and 7.8% lower end-to-end latency on real workload data with diverse input and output trends from Cloud Provider X. Additionally, the proposed framework can also serve as a standard for benchmarking different LLM inference schedulers since it provides the best latency for a given model, hardware, and instance-level scheduler combination.

==> sections/4_EmpiricalStudy.tex <==
\begin{figure*}
    \centering
        \begin{subfigure}{0.33\linewidth}
        \resizebox{\linewidth}{!}{%
         \input{plots/tikzplots/prompt_execution_time}
        }
        \caption{Effect of prompt length}\label{fig:prompt_length_execution_time}
    \end{subfigure}%
    \begin{subfigure}{0.33\linewidth}
        \resizebox{\linewidth}{!}{%
         \input{plots/tikzplots/decode_iteration_time}
        }
        \caption{Effect of  decode length}\label{fig:decode_length_execution_time}
    \end{subfigure}%
    \begin{subfigure}{0.33\linewidth}
        \resizebox{\linewidth}{!}{%
        \input{plots/tikzplots/spiking_example_cumsum}
        }
        \caption{Effect of request mixing}\label{fig:mixing_requestsv1}
    \end{subfigure}%
    \caption{\textbf{Effects of prompt and decode tokens on batch execution time.} (a) Execution time of batch with a request in prefill phase grows fast and linearly with the number of prefill tokens. (b) Execution time of batch with only decode tokens is affected to a much lesser degree with the number of tokens. (c) Increase in execution time on mixing requests with the arrival pattern of Figure \ref{fig:mixing_requests}  
    }
    \label{fig:mixing_overview}
\end{figure*}


\section{Observation}

\label{Sec: Observation}
\begin{table*}[t]
\adjustbox{max width=\textwidth}{%
    \centering
    \begin{tabular}{cccccccc}
        \hline
        \multirow{2}{*}{\textbf{Source}} & \multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Samples}} & \multicolumn{2}{c}{\textbf{Average Tokens}} & \multirow{2}{*}{\textbf{Heavy Decode}} & \multicolumn{2}{c}{\textbf{Accuracy}} \\
        & & & \textbf{Prompt} & \textbf{Decode} & & \textbf{SOTA} & \textbf{Ours} \\
        \hline
        Books~\citet{tiedemann-2012-parallel} & Translation & 7351 & 29.09 & 61.76 & 9.18\% & 4.47\% & 93.10\% \\
        
        Eli5 (Reddit subset)~\citet{eli5_lfqa} & QnA & 6988 & 29.83 & 334.40 & 58.18\% & 5.91\% & 70.36\% \\
        IMDb~\citet{maas-EtAl:2011:ACL-HLT2011} & Sentiment Analysis & 6564 & 211.54 & 142.53 & 41.01\% & 6.81\% & 79.92\% \\
        SQuAD~\citet{rajpurkar-etal-2016-squad} & In-context QnA & 7122 & 125.16 & 220.02 & 47.95\% & 6.22\% & 65.27\% \\
        WNUT~\citet{derczynski-etal-2017-results} & Entity Recognition & 3304 & 26.41 & 64.10 & 8.71\% & 2.76\% & 95.06\% \\
        \hline
        \textbf{Total} & - & 31329 & 89.03 & 175.71 & 35.54\% & 5.5\% & 79.15\% \\
        \hline
    \end{tabular}}
    \caption{\textbf{Dataset and Performance of Output Length Predictor.} Average prompt and decode tokens varies across data sources. The second last column indicates the percentage of requests with heavy decodes ($\geq 5$ seconds estimated completion time) and the last column indicates the accuracy of our decode length predictor model described in \autoref{sec:output_length_predictor} for each source.
    }
    \label{tab:dataset_distrib}
\end{table*}

\subsection{Prompt-Decode characteristics of requests and execution time} In general, LLM queries come from different tasks and  differ in terms of their prompt and decode distribution. We simulate this using data from five different tasks: sentiment analysis, entity recognition, in-context QnA, general QnA, and translation (prompt details in Appendix~\ref{app:dataset_details}). Table~\ref{tab:dataset_distrib} summarizes the distribution of input (prompt) and generated output (decode) tokens for the requests from these tasks. We see a clear distinction in the average length of prompt and decode tokens, and in the percentage of requests with heavy decode, across tasks.

Based on these observations, we divide requests into four categories: light prompt-light decode (LL), light prompt-heavy decode (LH), heavy prompt-light decode (HL), and heavy prompt-heavy decode (HH). Requests that take 0.5 seconds or more to complete their prompt phases are defined as heavy prompts, and requests that take 5 seconds or more in the decode phase are defined as heavy decodes. We make the division between heavy and light tokens based on latency as (i) latency is the key metric that we are optimizing in this work and (ii) they are representative of the SLAs that different service providers might have. These values are hyperparameters that can be tuned to the provider's needs.
{It is to be noted that the execution time (latency) varies from one hardware to different, so in order to have a common ground, we are using prompt and decode processing time to define light/heavy classification. }
\textcolor{blue}{I feel it is better to start with batch execution time for prompt and decode and then get into io classification. Batch execution time for prompt/decode > >need for IO classification based on execution time > >provides common ground for a framework applicable across models, hardware > > this is relevant as more and more hardware and models would come soon.}

Figures~\ref{fig:prompt_length_execution_time} and ~\ref{fig:decode_length_execution_time} show that batch execution time increases linearly with the number of prompt tokens due to it's compute bound nature, and the growth is much slower during the decode phase. Thus, we estimate the processing time for a request with $p$ prompt and $d$ decode tokens as {\color{black}$ p \times (\texttt{time per prompt token}) + d \times (\texttt{average decode batch time})$}. Similarly, the earliest time any model instance will become available is {\color{black}$(\texttt{decode tokens left})\times(\texttt{average decode batch time})$}. \textcolor{blue}{AP: to modify} 
In the following section, we discuss the impact of serving these requests concurrently on a single LLM instance and the effect of routing and scheduling logic on the end-to-end performance of inference across multiple model instances.

% \subsection{Effects of Mixing Requests} 
\subsection{Mixing inference requests on a single model instance can harm latency and end-to-end performance} 
The unique characteristics of LLM requests causes the end-to-end latency to be adversely affected by continous batching of requests. For example, the ideal latency for a request with $p=1000$ and $d=1000$ is $17$ seconds (orange plot in Figure \ref{fig:mixing_requestsv1}). However if we now have requests with $p=500$ and $d=500$ arriving and getting batched with this request at every $50^{\mbox{th}}$ iteration then the end-to-end latency of the original request goes up to 31 seconds (Figures \ref{fig:mixing_requests} and \ref{fig:mixing_requestsv1}). This is due to the latency spikes caused by the prompt phase of each of the incoming requests due to which the latency of the original request goes up even though the decoding happens in parallel. The additional latency spikes in the prompt phase differentiates LLM inference from other batch jobs. 

\begin{table*}
\adjustbox{max width=\textwidth}{%
    \centering
    \begin{tabular}{cccccc}
        \hline
        \multirow{2}{*}{\textbf{Batching Algorithm}} & \multirow{2}{*}{\textbf{Routing Algorithm}} & \multicolumn{4}{c}{\textbf{Total End to End Latency (seconds)}} \\
        \cmidrule(lr){3-6}
        & & \textbf{(LH, HL random)} & \textbf{(Random)} & \textbf{(LH, then HL)} & \textbf{(HL, then LH)} \\
        \hline
        \multirow{3}{*}{Bin Packing~\citet{jin2023s3}} & Dedicated Small-Large & 704.5 & 644.75 & 566.25 & 588.15 \\
        & Round Robin & \textbf{581.5} & 559.3 & 424.8 & \textbf{440.68} \\
        & Decode Balancer & 595.82 & 555.4 & 424.82 & 440.81 \\
        \hline
        \multirow{3}{*}{Least Work Left} & Dedicated Small-Large & 704.5 & 641.81 & 566.25 & 588.15 \\
        & Round Robin & 585.14 & \textbf{554.00} & \textbf{424.64} & 440.82 \\
        & Decode Balancer & 596.95 & 559.97 & 424.66 & 440.81 \\
        \hline
        \multirow{3}{*}{FCFS~\citet{orca}} & Dedicated Small-Large & 704.5 & 648.66 & 566.25 & 588.15 \\
        & Round Robin & 607.45 & 572.16 & 424.80 & 440.82 \\
        & Decode Balancer & 605.65 & 573.17 & 424.82 & 440.81 \\
        \hline
    \end{tabular}}
    \caption{\textbf{Performance of batching and routing algorithm combinations.} We simulate arrival of requests with distinct characteristics  using the request classification discussed in ~\autoref{Sec: Observation} and test the combined affect of routing and batching strategies. 
    Good routing algorithm on an average shows greater end-to-end latency improvement compared to the batching algorithm on all the scenarios with distinct characteristics and arrival sequence. 
    }
    \label{tab:batching_routing_combo}
\end{table*}

\subsection{The end-to-end latency is affected by the request arrival patterns and both the routing and the batching algorithms}
% \subsection{Factors affecting E2E Latency}
% The end-to-end latency is affected by the request arrival patterns and both the routing and the batching algorithms.
To understand the effect of routing on the overall end-to-end latency of the system, we take two LLM instances and consider the following arrival patterns of 3000 requests: 1) LH and HL requests arriving in a random fashion, 2) Requests from all four classes arriving in a random fashion, 3) LH requests arriving first followed by HL requests, and 4) HL requests arriving first followed by LH requests. We study the end-to-end latency in each scenario with different combinations of batching and routing algorithms. Details of these algorithms are added to Appendix \ref{app:heuristic}. We can see from Table \ref{tab:batching_routing_combo} that it is the combination of routing and batching algorithms that affects the overall end-to-end latency of processing the requests. 

For example, the bin-packing scheduler finishes Scenario I six seconds faster when using round-robin routing compared to decode balancer routing but the same combination is four seconds slower when benchmarked on Scenario II. We also observe that sub-optimal routing strategies, such as having dedicated servers for small and large requests, can have a severely adverse effect on the overall performance of our system. This highlights the importance of optimizing the routing strategy and shows that scheduling algorithms can only provide results as good as the choices provided to it by the router.

Another interesting insight is that, for Scenario IV, all the batching algorithms show the exact same end-to-end latency, and it is the routing algorithm that improves the end-to-end latency. This is because, regardless of selecting batching algorithms such as Least Work Left, the requests coming in first have a low number of decode tokens and are thus affected less by incoming prompt tokens, which are themselves quite light. 
This indicates the dependence of performance on the arrival sequence of requests with different characteristics.

\subsection{Insights} Quantitative analysis 
highlights the importance of considering request characteristics and avoiding serving requests with diverse characteristics concurrently at a single LLM instance, especially when multiple LLM instances are available.
Further, the routing algorithm on an average shows greater end-to-end latency improvement compared to the batching algorithm on all the scenarios with distinct characteristics and arrival sequence. 
We propose to optimize routing logic for a given batching algorithm and workload characteristics. A data-driven optimal router framework can translate the improvements to any downstream batching logic.
% \TODO{revisit the structure of this section and reorder if needed after we finalize Section 4.}
Anchoring on our thesis that batching algorithm can only provide results as good as the choices provided to it, in the next section, we propose a workload-aware intelligent router and discuss the overall design of the router and the individual building blocks required.


